ToolTango: Common sense Generalization in Predicting Sequential Tool Interactions for Robot Plan Synthesis

Robots assisting us in environments such as factories or homes must learn to make use of objects as tools to perform tasks, for instance using a tray to carry objects. We consider the problem of learning commonsense knowledge of when a tool may be useful and how its use may be composed with other tools to accomplish a high-level task instructed by a human. Specifically, we introduce a novel neural model, termed TOOLTANGO, that first predicts the next tool to be used, and then uses this information to predict the next action. We show that this joint model can inform learning of a fine-grained policy enabling the robot to use a particular tool in sequence and adds a significant value in making the model more accurate. TOOLTANGO encodes the world state, comprising objects and symbolic relationships between them, using a graph neural network and is trained using demonstrations from human teachers instructing a virtual robot in a physics simulator. The model learns to attend over the scene using knowledge of the goal and the action history, finally decoding the symbolic action to execute. Crucially, we address generalization to unseen environments where some known tools are missing, but alternative unseen tools are present. We show that by augmenting the representation of the environment with pre-trained embeddings derived from a knowledge-base, the model can generalize effectively to novel environments. Experimental results show at least 48.8-58.1% absolute improvement over the baselines in predicting successful symbolic plans for a simulated mobile manipulator in novel environments with unseen objects. This work takes a step in the direction of enabling robots to rapidly synthesize robust plans for complex tasks, particularly in novel settings

==> platform.tex <==
\section{Data Collection Platform}

\textbf{Robot Actions.} 
We consider non-dexterous manipulation and planar navigation platforms. Later,  the framework can be extended to agile platforms that can jump or fly through. These platforms can execute human-understandable behaviours. Note that since our work focuses on long range actions rather than very local skills, the robot behaviours may not be physically simulated, it will suffice to show their coarse effects on the environment. 

\begin{table}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c||c|c|}
    \hline 
    \textbf{Objects} & \begin{minipage}[t]{0.63\columnwidth}Each object is represented as a URDF model. Objects have a location,
    spatial extent, properties such as types and can be placed on/inside
    others.\end{minipage}  & \begin{minipage}[t]{0.63\columnwidth}Tray, box, fruits, table, ramp, barrier, bridge like item, light switch,
    Rigid blocks of different sizes, walls, door, window, ground plane
    (may have gaƒps).\end{minipage} \tabularnewline
    \hline 
    \textbf{Regions} & \begin{minipage}[t]{0.63\columnwidth}Associate canonical region of space with objects such as the region
    that is on the table or the left side as they may be referenced in
    language.\end{minipage} & Region on the table, region on the ground etc.\tabularnewline
    \hline 
    \textbf{Robots} & \begin{minipage}[t]{0.63\columnwidth}We start with a mobile manipulator capable of non-dexterous manipulation.\end{minipage} & Husky + UR5 arm\tabularnewline
    \hline 
    \end{tabular}}
    \caption{World Composition in simulator}
    \label{tab:world_composition}
\end{table}

\begin{table}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|}
    \hline 
    \textbf{World aspects} & \textbf{Description} & \textbf{Potential Sources}\tabularnewline
    \hline 
    \hline 
    Geometric attributes & \begin{minipage}[t]{0.53\columnwidth}Location, IsMovable, Flatness (ratio of width to height), Size\end{minipage} & Form perception/simulation or basic object geometry\tabularnewline
    \hline 
    Geometric relations & \begin{minipage}[t]{0.53\columnwidth}Relative spatial relations such as size or OnTop(if an object is on
    top of another).\end{minipage}  & From perception/simulation.\tabularnewline
    \hline 
    Semantic attributes & \begin{minipage}[t]{0.53\columnwidth}Object type and ontologies and unary properties. Labels such as \textquotedblleft box\textquotedblright ,
    \textquotedblright apple\textquotedblright , \textquotedblleft fruit\textquotedblright{}
    or made\_of (cardboard)\end{minipage} & From ConceptNet\tabularnewline
    \hline 
    Relative semantic properties & \begin{minipage}[t]{0.53\columnwidth}Relative strengths/rigidness/expected sizes.\end{minipage} & From VerbPhysics\tabularnewline
    \hline 
    Global variables properties
     & Lights on/off & Encoded in simulation. \tabularnewline
    \hline 
    \end{tabular}}
    \caption{Properties of object in the simulated world}
    \label{tab:properties}
\end{table}

\paragraph{World Representation.} We take a multiverse view of the world where the world can be represented in a hybrid symbolic-metric space. Our world is object centric but we imbue both metric and semantic properties to them (Table~\ref{tab:world_composition}). The state consists of variables that model the named aspects of the world (Table~\ref{tab:properties}). These are derived from direct observations of the world and background knowledge. 


\subsection{Simulator Assumptions and Implementation}

We need a low-fidelity visualization/simulation environment where the robot can take actions and interact. The low-level physics of motion is less important, we are primarily concerned with the symbolic effects on the world state. We present the human agents with a scene and a goal state we want to attain and they either use an interface to give us actions or use language to describe what they want. The language instruction will be grounded in the world and the agent and the virtual environment will show its effects. 


\begin{figure}[!t]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/simulator/setup.PNG}
    \caption{\footnotesize \textbf{Environment model} for determining robot actions given the current world state, instruction indicative of the goal state and existing semantic knowledge. }
    \label{fig:env_model}
\end{figure}

The agent model for determining robot actions given the current world state is given in Figure~\ref{fig:env_model}. Instruction indicative of the goal state and existing semantic knowledge. Note that we aim to learn a model that predicts actions on how the robot can connect the current and the future state say be using an object as a tool etc. A data set is collected consisting of  traces with actions provided by the human. This data set is used to learn to predict actions. The intuition is that the model should be able to learn the commonsense about object types and primitive physical properties of the objects in the environment context. 


To allow such actions to be executed and for symbolic level physics management, we compared various simulators and realized that the PyBullet  (based on \emph{Bullet} physics engine by~\cite{coumans2016pybullet}) allows most simplistic implementations of actions, relations and object manipulation regions and hence was chosen as our simulator.

\subsection{Action Implementation}

There are two types of actions:

\begin{compactenum}
    \item \textbf{Interpretable symbolic actions:} The human instructs the robot by selecting interpretable symbolic actions.  Format for mobile manipulation: Move(robot, object, base) where the robot moves an object to a base where the base can be another object or a region.  The user will select the operators based on objects available. In the next phase we can allow the user to enter language descriptions. In that case, the language would be grounded into a structured format. Formally, an action such as Move(robot, object, base) can be interpreted as the following constraints:
    \begin{itemize}
        \item A set of goal constraints that the robot should achieve at the end of the action such that say an apple should be on the tray. 
        \item A set of motion constraints that may be active during the motion such as for slide, the robot should always keep the object it is pushing on the ground.
        \item These constraints will serve as inputs to the robot controller that can synthesize the motion plan to accomplish the indicated goals while respecting the specified constraints during the motion. 
    \end{itemize}
    Symbolic actions include: \begin{lstlisting}
        pick and place, move to, push, climb up/down, place on, drop to, change state, place ramp, stick, fuel, cut, print, drive, drill, apply and clean. 
    \end{lstlisting}
    \item \textbf{Sub-symbolic actions:} A symbolic action is executed as short sequences of low-level operators. Each has a name and conditions when it is active and its effects. The planning process can connect the operators.  For simple mobile manipulation the operators are listed below for discussion. 
\end{compactenum}

 Also, please note that for this work, we are operating in a discretized world of objects and regions. Hence, a reference to a continuous quantity such as a pose means referring to an object or a fixed location where the robot goes. Similarly, a final pose for the robot means a canonical pose that it goes to after picking or placing an object. 
 
\subsection{Object Relation Implementation}

Any world having objects must have some semantic relations among them. Examples of relations can include: on top, inside and whether the object is reachable from the robot or not. Some examples of different relations are given below.

\begin{compactenum}
    \item \textbf{Establish containment}:
    \begin{itemize}
       \item Contain: Books - box
       \item Contain: Fruits - tray
       \item Contain: Small items - small box
       \item Contain: Trash - garbage box
    \end{itemize}
    \item \textbf{Establish contact (rigid joint)}
    \begin{itemize}
       \item Connecting Dirt - mop
       \item Connecting Nail - wall
       \item Connecting Dirt - cloth
    \end{itemize}
    \item \textbf{Stable pushing}
    \begin{itemize}
       \item Push/slide: box
       \item Push away: obstructions/blocks
    \end{itemize}
    \item \textbf{Connect parts of the state space}
    \begin{itemize}
        \item Connecting with horizontal block
        \item Connecting vertically with ramps, staircases, jump platforms.
    \end{itemize}
    \item \textbf{Actions with continuous dynamics}
    \begin{itemize}
        \item Drop an item in a box
        \item Hitting a nail with a hammer
        \item Throw an object
    \end{itemize}
    \item \textbf{Stable support} like placing a tray on the table before using the manipulator for an alternative task. 
\end{compactenum}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/simulator/manipulation_region.pdf}
    \caption{Manipulation region of an object}
    \label{fig:manipulation_region}
\end{figure}
 
To implement various relations among objects PyBullet allows to define \emph{manipulation regions} around objects. These regions are virtual regions inside which a robot can manipulate that object. A visual description of this region is shown in Figure~\ref{fig:manipulation_region}.

We now define two object types.
\begin{compactenum}
    \item \textbf{Standalone object:} Such an object is defined as a collection of stereo-lithographic tetrahedrons with visual and collision properties. Each such object has a single manipulation region, denoted as $MR(object)$, which is the region around the object where it is considered to be in ``vicinity'' to the object and hence can be manipulated by the robot. Ex: cubes, fruits, milk, etc.
    \item \textbf{Containing object:} Such an object is a standalone object with an additional containment region, denoted as $CR(object)$, which is a proper subset of the manipulation region where if another object’s center lies is called to be “contained inside” this object. Ex: box, cupboard and fridge.
\end{compactenum}

Every object has a center defined arithmetic mean of the centers of the tetrahedrons, denoted by $C(object)$. We now define the two relation constraints of which others are different versions of combinations of:

\begin{compactenum}
    \item \textbf{Inside:} An object $A$ is said to be contained inside a containing object $B$ if the $C(A) \in CR(B)$.
    \item \textbf{On Top:} An object $A$ is said to be on top on another object $B$ if $C(A)_z > C(B)_z$ and $MR(A) \cap MR(B) \neq \phi$, where $C(O)_z$ denotes the z component of the center of object $O$.
\end{compactenum}


\subsection{User Interface}

The interface that was used to collect data is shown in Figure~\ref{fig:simulator}. The PyBullet camera stream was sent to the simulator using Flask library. Flask is a micro web framework written in Python. It is classified as a micro-framework because it does not require particular tools or libraries. It has no database abstraction layer, form validation, or any other components where pre-existing third-party libraries provide common functions. However, Flask supports extensions that can add application features as if they were implemented in Flask itself. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/screenshot2.png}
    \caption{
    \footnotesize{\textbf{Data collection platform.} 
    The human teacher instructs the virtual mobile manipulator robot 
    by specifying symbolic actions. The human-instructed plan is then simulated and visualized using the interface.}
    }
    \label{fig:simulator}
\end{figure}

% The interface consists of object set with exploration on click, i.e. when an object is clicked, the interface shows the image of the object with its vicinity. A human user can also rotate and zoom in the third-person camera. An action input drop-down allows user to enter actions to the interface input. `Execute' and `Undo', allow executing the input action or undoing the last executed action.

The user interface required many iterations and innovations in order to be able to collect data from human teachers in an efficient manner. In the following subsections, we list out the design choices made while realizing this interface.

\subsection{Design of the environment}

While designing the environment it was important that the simulated environment looks quite close to what a home or a factory actually looks like. The objects present should also look as they would look in the real world. Our simulator is heavily based on object interactions and we also simulate the physics of the environment, thuds the models for these objects need to be constructed very carefully.

The objects in the domains were derived from real-world home and factory scenes that span Facebook Replica Dataset \cite{DBLP:journals/corr/abs-1906-05797}. These scenes were made to look as photo realistic as possible. The objects on other other hand were chosen to span the YCB dataset \cite{calli2017ycb} with the STL file for each object constructed from the ground up, from basic mechanical engineering principles. This was done in order to keep the simulated physics as real as possible. Small aberrations in this STL file could lead to objects behaving unnaturally. We provide a list of the objects in the home and factory domain in Table~\ref{tab:env_desc1}

\begin{table}
    \centering
    \resizebox{0.8\textwidth}{!}{
    \begin{tabular}{|c|}
    \toprule 
    \textbf{Home Objects}\tabularnewline
    \midrule 
    \begin{minipage}[t]{0.93\columnwidth}floor$^{1}$, wall, fridge$^{123}$, cupboard$^{123}$, tables$^{1}$, couch$^{1}$, \textbf{big-tray}$^{1}$, \textbf{tray}$^{1}$, \textbf{book}$^{1}$,
    paper, cubes, light switch$^{4}$, bottle, \textbf{box}$^{2}$, fruits, \textbf{chair}$^{15}$, \textbf{stick}, dumpster$^{2}$,
    milk carton, shelf$^{1}$, \textbf{glue}$^{6}$, \textbf{tape}$^{6}$, \textbf{stool}$^{15}$\tablefootnote{Stool/ladder are proxies for raising the height of the robot}, \textbf{mop}$^{8}$, \textbf{sponge}$^{8}$, \textbf{vacuum}$^{8}$, dirt$^{7}$, door$^{2}$\end{minipage}\tabularnewline
    \midrule
    \textbf{Factory Objects}\tabularnewline
    \midrule 
    \begin{minipage}[t]{0.93\columnwidth}floor$^{1}$, wall, \textbf{ramp}, worktable$^{1}$, \textbf{tray}$^{1}$, \textbf{box}$^{2}$, crates$^{1}$, \textbf{stick}, long-shelf$^{1}$,
    \textbf{lift}$^{1}$, cupboard$^{123}$, \textbf{drill}$^{4}$, \textbf{hammer}$^{49}$, \textbf{ladder}$^{5}$, \textbf{trolley}$^{2}$, \textbf{brick}, \textbf{blow dryer}$^{48}$,
    \textbf{spraypaint}$^{4}$, \textbf{welder}$^{4}$, generator$^{4}$, \textbf{gasoline}, \textbf{coal}, \textbf{toolbox}$^{2}$, \textbf{wood cutter}$^{4}$,
    \textbf{3D printer}$^{4}$\tablefootnote{3D printer is a proxy for known but unobserved objects}, screw$^{9}$, nail$^{9}$, \textbf{screwdriver}$^{49}$, wood, platform$^{1}$, oil$^{7}$, water$^{7}$,
    board, \textbf{mop}$^{8}$, paper, \textbf{glue}$^{6}$, \textbf{tape}$^{6}$, assembly station, spare parts, \textbf{stool}$^{15}$\end{minipage}\tabularnewline
    \bottomrule 
    \end{tabular}}
    \caption{\footnotesize{\textbf{Domain Representation. } The different objects present in the home and factory domain along with their properties. Legend:- $^{1}$:~surface, $^{2}$:~can open/close, $^{3}$:~container, $^{4}$:~can operate, $^{5}$:~can climb, $^{6}$:~can apply, $^{7}$:~can be cleaned, $^{8}$:~cleaning agent, $^{9}$:~can 3D print.}}
    \label{tab:env_desc1}
\end{table}

\subsection{Human Aspect of the Design}

As the interface had to finally be used by humans who are not versed in the intricacies of robotics, it was necessary that the interface is easy to use and intuitive for these users. Thus, we collected feedback from users to improve the interface at each iteration.

First, users faced difficulties in understanding the environment. This is because the human cannot understand how the simulator exactly works and the large space of actions makes it difficult for him to appreciate what all the robot can accomplish. Thus, taking inspiration from the interactive tutorials present in video games where the user is put in a simpler environment, we constructed relatively simple goals which are easier for the user to accomplish (Figure~\ref{fig:tutorial}). In addition to these tutorials, the user was also asked to see a video before each goal, which helped him appreciate the interactions that he could use to accomplish the next goal. Having gained experience and confidence from completing the tutorial, the user was able to give better data for our task.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/simulator/tutorial.PNG}
    \caption{
    \footnotesize{\textbf{Tutorial.} A user friendly tutorial for human demonstrators.}
    }
    \label{fig:tutorial}
\end{figure}

Second, it was not intuitive for the users that they need to give optimal plans for the robot to complete. They have a tendency to ``play'' with the simulator at the start of the data collection, using useless actions to complete the plan. Thus it was necessary for us to prime the user, by spelling out explicitly that we want to the plans given by the users to be optimal. In addition, we also added a count down timer to the interface, which puts artificial pressure on the user to complete plans quickly.

Third, it was found that the first round of data collection yielded low number and quality of datapoints. However, once the serious users from the first round of data collection are identified, due to the familiarity with the system the quality and number of datapoints received progressively increased.

Fourth, it was realized that the users find it difficult to understand that the robot has only one gripper as they were primed for two hands possessed by humans. Thus, it was important to explicitly spell this out in the interface to prevent them from giving extraneous commands.

\subsection{Visual Interface Design}

The users found it difficult to identify some objects or were not able to appreciate the wide range of objects that could be used to complete a task. For this reason, we added an explore button for each object in the scene, which on clicking would show you where exactly in the scene it is present. This increased the different objects that were utilized by users to complete goals, sometimes using objects that were not even anticipated while design of the interface.

We use a third person view of the environment instead of a first person view. This is because we require a broader worlds view of all objects. A first person view limited the vision of the robot, and thus limited the user from improvising with completely new objects.
It was identified that the process of giving commands is usually easier and takes place faster than the commands actually being performed. Thus we made the process of giving commands asynchronous from the actual robot operation. The given operations were appended to a queue of instructions which the robot pops and completes.

\subsection{Optimizations for the End User}

The user interface needs to run on a browser that an end user utilizes. This means that the amount of computation that can be done on the client side is limited by the hardware present with him. The graphic card requirements for running PyBullet may be difficult to obtain for most users. Thus, we moved to client-server model where all physics computation and graphic simulation is done by the server, and the result is sent to the client.

However, sending the entire simulator state is wasteful and can put unnecessary load on the network bandwidth. In order to reduce the communication overhead, we run the PyBullet simulator on the server but only send images of the simulated environment to the client at short and regular intervals. We use Flask in order to show this stream of photos to the user. In order to speed up the simulation process, we do not render the RGB graphics of the PyBullet simulator and run it in a headless mode, directly taking photographs of the simulator. This reduces the time taken to simulate the actions as the graphic rendering overhead is reduced.

\subsection{Interaction among platform components}

To interact with the interface, the human either clicks or provides instructions that are received by a GUI interface that sends the corresponding symbolic action to the robot controller. The robot controller expresses the symbolic actions into sub-symbolic actions based on the environment state which is then executed on the robot. The world state is stored in the world model which any component can access. The series of steps to generate a datapoint are given below.

\begin{compactenum}
    \item The simulator generates a random goal-scene pair.
    \item The simulator sends scene and goal specification to UI.
    \item The UI grounds goal natural language text
    \item UI reders scene using Flask library.
    \item User inputs high level action.
    \item UI does language and semantic grounding.
    \item UI sends symbolic actions to simulator.
    \item The world simulator decomposes symbolic actions to sub-symbolic actions.
    \item Simulator performs constraint checking.
    \item The simulator calculated trajectory and generates motion plan.
    \item The PyBullet engine executes the trajectories after physics constraint checking.
    \item The world simulator gets new state from the PyBullet engine.
    \item Simulator updates the world state and performs goal checking.
    \item The updated world state image and goal success is sent to interface.
    \item The above steps are looped till goal not reached.
\end{compactenum}

A characteristic datapoint is shown below for Factory domain and goal as `switch on generator'. The complete datapoint with sub-symbolic actions and state parameters can be seen in Appendix~\ref{appendix:world_scenes}. A video demonstrating the working of the simulated plan can be viewed at \url{https://youtu.be/-mIQuM3kjF4}.
\begin{lstlisting}
World = world_factory9
Goal = goal4-generator-on
Symbolic actions:
{'name': 'placeRamp', 'args': []}
{'name': 'moveTo', 'args': ['gasoline']}
{'name': 'pick', 'args': ['gasoline']}
{'name': 'moveUp', 'args': []}
{'name': 'fuel', 'args': ['generator', 'gasoline']}
{'name': 'drop', 'args': ['gasoline']}
{'name': 'changeState', 'args': ['generator', 'on']}.
\end{lstlisting}


\subsection{Dataset Creation From Human Demonstrations}
\label{sec:data_collection}

%
Our goal is to learn common sense knowledge about tool usage from 
human teachers instructing the robot to attain declarative goals. 
%
We proceed by creating a physics simulation environment to model a mobile manipulator\footnote{a Universal Robotics Manipulator (UR5) mounted on a Husky mobile base} capable of executing symbolic actions for a diverse range of tasks.  
%
We then use the environment to collect a data set of human demonstrations that instruct the robot to perform tasks in the environment.  

\subsection{Virtual Environment and User Interaction}

%
A simulation environment using PyBullet was used to encode a home-like and a factory-like domain. 
%
A virtual mobile manipulator could pursue the following categories of semantic goals: (a) 
\emph{transporting} objects from one region to another (including space on top of or inside 
other objects), (b) \emph{fetching} objects where the robot must reach, grasp and return with, and (c) \emph{inducing state changes} such as illuminating the room or removing dirt on the floor.  
%
% \blue{
% \begin{itemize}
% \item Say that there were X instances, Y objects.
% \item Need to say that the scenes and the objects used were based on a standard scene layout. Not cherry picked. 
% Important to say that we have not been (too) biased in our creation of the data set. 
% \item Refer to table of actions and Figure of goals
% \end{itemize}
% }
%
The robot's interactions were implemented with a 
low-level motion planner with a set of encoded discrete conditions 
such as moving close to an object before manipulating etc. arising 
due to physical constraints of the robot. 
%
The set of abstract interactions such as attachment, operating a tool or specifics of grasping 
were encoded symbolically as the establishment or release of constraints. 
%
The effects of actions such as pushing, moving and contact with a stick-like object 
were simulated and propagated to the next time step. 
%
Two domains of home and factory were implemented with objects as states in Table~\ref{tab:env_desc}. 
%
The objects in the domains were derived from real-world home and factory scenes and diverse object types that span Facebook
Replica Dataset (\citet{straub2019replica}) and YCB object dataset (\citet{calli2017ycb}).
%
For each domain, 8 different goals were given to human instructors as stated in Table~\ref{tab:dataset}.
% 
A lexical parser was built to convert goal specification to constraints on the state of the simulator.
%
Moreover, 10 different scenes for each domain were created by randomly positioning different objects 
based on likely semantic placements. 
%
For instance, fruits could be placed $\mathrm{OnTop}$ of table or $\mathrm{Inside}$ the fridge.

A human instructor could interact with the robot agent by selecting a goal and 
specifying a sequence of symbolic action to execute. 
%
The specified plan was then simulated showing the robot interacting 
with objects and changing the world state. 
%
The human subjects are encouraged to instruct the robot such that the task 
is completed as quickly as possible, making use of available tools in the environment. 
%most efficient plans to accomplish the 

\subsection{Dataset Characteristics}
\begin{table}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline 
    \multirow{2}{*}{Domain} & \multirow{2}{*}{Plan lengths} & Objects interacted & Tools used & \multirow{2}{*}{Objects} & \multirow{2}{*}{Goal specifications}\tabularnewline
     &  &  with in a plan & in a plan &  & \tabularnewline
    \hline 
    \hline 
    Home & 23.25$\pm$12.65 & 4.12$\pm$1.97 & 0.93$\pm$0.70 & \begin{minipage}[t]{0.7\textwidth}floor$^{1}$, wall, fridge$^{123}$, cupboard$^{123}$, tables$^{1}$, couch$^{1}$, \textbf{big-tray}$^{1}$, \textbf{tray}$^{1}$, \textbf{book}$^{1}$,
        paper, cubes, light switch$^{4}$, bottle, \textbf{box}$^{2}$, fruits, \textbf{chair}$^{15}$, \textbf{stick}, dumpster$^{2}$, milk carton, shelf$^{1}$, \textbf{glue}$^{6}$, \textbf{tape}$^{6}$, \textbf{stool}$^{15}$\tablefootnote{Stool/ladder are proxies for raising the height of the robot}, \textbf{mop}$^{8}$, \textbf{sponge}$^{8}$, \textbf{vacuum}$^{8}$, dirt$^{7}$, door$^{2}$\end{minipage} & \begin{minipage}[t]{0.4\textwidth} 1. Place milk in fridge, 2. Place fruits in cupboard, 3. Remove dirt from floor, 4. Stick paper to wall, 5. Put cubes in box, 6. Place bottles in dumpster, 7. Place a weight on paper, 8. Illuminate the room. \vspace{2pt}
        \end{minipage}\tabularnewline
    \hline 
    Factory & 38.77$\pm$23.17 & 4.38$\pm$1.85 & 1.44$\pm$0.97 & \begin{minipage}[t]{0.7\textwidth}
        floor$^{1}$, wall, \textbf{ramp}, worktable$^{1}$, \textbf{tray}$^{1}$, \textbf{box}$^{2}$, crates$^{1}$, \textbf{stick}, long-shelf$^{1}$, \textbf{lift}$^{1}$, cupboard$^{123}$, \textbf{drill}$^{4}$, \textbf{hammer}$^{49}$, \textbf{ladder}$^{5}$, \textbf{trolley}$^{2}$, \textbf{brick}, \textbf{blow dryer}$^{48}$,
        \textbf{spray-paint}$^{4}$, \textbf{welder}$^{4}$, generator$^{4}$, \textbf{gasoline}, \textbf{coal}, \textbf{toolbox}$^{2}$, \textbf{wood cutter}$^{4}$, \textbf{3D printer}$^{4}$\tablefootnote{is a proxy for known but unobserved objects}, screw$^{9}$, nail$^{9}$, \textbf{screwdriver}$^{49}$, wood, platform$^{1}$, oil$^{7}$, water$^{7}$,
        board, \textbf{mop}$^{8}$, paper, \textbf{glue}$^{6}$, \textbf{tape}$^{6}$, assembly station, spare parts, \textbf{stool}$^{15}$\vspace{2pt}\end{minipage} & \begin{minipage}[t]{0.4\textwidth} 1. Stack crated on platform, 2. Stick paper to wall, 3. Fix board on wall, 4. Turn on the generator, 5. Assemble and paint parts, 6. Move tools to workbench, 7. Clean spilled water, 8. Clean spilled oil. \vspace{2pt}
        \end{minipage}\tabularnewline
    \hline 
    \end{tabular}}
    \caption{\footnotesize{\textbf{Dataset characteristics:} Average plan lengths, number of objects interacted in plan and number of tools used in plans with object and goal sets for Home and Factory domains. Legend:- $^{1}$:~surface, $^{2}$:~can open/close, $^{3}$:~container, $^{4}$:~can operate, $^{5}$:~can climb, $^{6}$:~can apply, $^{7}$:~can be cleaned, $^{8}$:~cleaning agent, $^{9}$:~can 3D print. Objects in bold can be used as tools.}}
    \label{tab:dataset_complete}
\end{table}

\begin{table}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cccccc}
    \toprule 
    Goal ID & Goal Text & Actions & Time & Interacted Objects & Tools used\tabularnewline
    \midrule
    \multicolumn{6}{c}{Home Domain}\tabularnewline
    \midrule
    1 & Place milk in fridge & 5.15$\pm$2.14  & 40.03$\pm$0.04  & 3.11$\pm$1.04 & 0.62$\pm$0.70\tabularnewline
    2 & Put fruits in cupboard & 5.15$\pm$1.72  & 48.04$\pm$0.03 & 4.69$\pm$1.10 & 0.60$\pm$0.57\tabularnewline
    3 & Remove dirt from floor & 4.26$\pm$1.10  & 18.21$\pm$0.01 & 3.33$\pm$0.91 & 1.43$\pm$0.51\tabularnewline
    4 & Stick paper to wall & 4.31$\pm$2.19 & 41.29$\pm$0.02 & 4.41$\pm$1.17 & 1.38$\pm$0.51\tabularnewline
    5 & Put cubes in box & 6.47$\pm$2.61 & 66.80$\pm$0.06 & 6.25$\pm$1.18 & 0.79$\pm$0.67\tabularnewline
    6 & Place bottles in dumpster & 7.46$\pm$2.02 & 313.92$\pm$0.12 & 6.99$\pm$1.10 & 1.24$\pm$0.72\tabularnewline
    7 & Place a weight on paper & 2.07$\pm$1.59  & 33.06$\pm$0.04 & 2.69$\pm$0.95 & 0.70$\pm$0.63\tabularnewline
    8 & Illuminate the room & 3.17$\pm$1.85  & 13.29$\pm$0.01 & 1.77$\pm$0.62 & 0.64$\pm$0.50\tabularnewline
    \midrule
    \multicolumn{6}{c}{Factory Domain}\tabularnewline
    \midrule 
    1 & Stack crates on platform & 12.59$\pm$2.42 & 745.55$\pm$0.46 & 5.71$\pm$0.99 & 1.37$\pm$0.75\tabularnewline
    2 & Stick paper to wall & 8.79$\pm$2.80 & 495.48$\pm$0.11 & 4.74$\pm$1.35 & 1.76$\pm$0.87\tabularnewline
    3 & Fix board on wall & 12.35$\pm$3.41 & 638.54$\pm$0.29 & 4.73$\pm$0.94 & 2.08$\pm$0.87\tabularnewline
    4 & Turning the generator on & 9.10$\pm$2.03 & 449.01$\pm$0.09 & 3.15$\pm$0.90 & 0.74$\pm$0.72\tabularnewline
    5 & Assemble \& paint parts & 22.60$\pm$5.31 & 1027.33$\pm$0.83 & 7.31$\pm$1.38 & 2.82$\pm$0.87\tabularnewline
    6 & Move tools to workbench & 8.47$\pm$1.80 & 514.79$\pm$0.21 & 4.54$\pm$0.99 & 0.73$\pm$0.67\tabularnewline
    7 & Clean spilled water & 4.73$\pm$1.94 & 247.90$\pm$0.31 & 2.46$\pm$0.56 & 1.05$\pm$0.22\tabularnewline
    8 & Clean spilled oil & 5.11$\pm$1.72 & 361.17$\pm$0.37 & 2.44$\pm$0.57 & 1.01$\pm$0.10\tabularnewline
    \bottomrule 
    \end{tabular}}
    \caption{\footnotesize{\textbf{Dataset characteristics. } The average number of actions, the mean object interactions and tools used for plans with associated goals for the human demonstrated robot plans collected in the home and factory domains. }}
    \label{tab:dataset}
\end{table}



The dataset was collected from human instructors by presenting different $\mathrm{goal,scene}$ pairs. The world scenes in object-centric graphs representation are shown in Appendix~\ref{appendix:world_scenes}.
% 
For each domain, every goal was combined with each scene to give $8\times10=80$ such pairs.
%
For each pair, 8 to 12 plans were collected based on the level of complexity and possible plan diversity. Objects sets, goal descriptions and other characteristics are shown in Table~\ref{tab:dataset_complete}. 
%
From 12 instructors, a complete set of $\mathrm{708}$ plans for home and $\mathrm{784}$ plans for factory domain were collected.
%
The original set of human demonstrated robot plans provides a limited set of environment contexts in which the plan 
are feasible. 
%
We augment the original set of demonstrations by exploring successful plans in perturbed environment contexts. 
%
Two plan augmentation strategies were used. Firstly, the plans that were successful for a goal in a 
world scene were tested on other scenes and were added to the dataset if on execution they lead
to the goal state in the simulated environment.
%
Secondly, we created more plans by randomly removing up to 5 objects that
are neither in the goal description nor interacted with in the plan.
%
After augmentation, the training datasets consist of $\mathrm{3540}$ 
and $\mathrm{3920}$ plans for home and factory, respectively.


Our dataset contains activities with several examples. 
%
Table~\ref{tab:dataset} analyzes the plan diversity and shows the variation of 
actions, total plan simulation time, number of interacted 
objects and tools with goals in each domain. 
Figure~\ref{fig:tool_with_goals} shows the
distribution of tool usage with different goals.
%
The frequency distribution of tool usage varies significantly with goals as different tools
are required to perform different activities. 
%
Different tools were used by human demonstrators for the same goal. 
%
Furthermore, placement of objects changes the tool usage distribution. For instance, a tray closer to
fruits is more likely to be chosen by a human instructor compared to a box far away. Figure~\ref{fig:plan_len} shows the number of plans for different plan lengths. Figure~\ref{fig:num_int} and \ref{fig:num_actions} show number of interactions with 10 most interacted objects and frequency of 10 most frequent actions respectively.

\begin{figure}[!b]
    \centering
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/toolnet/home_goal_tools.pdf}
        \caption{Home domain}
        \label{fig:home_goal_tools}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/toolnet/factory_goal_tools.pdf}
        \caption{Factory domain}
        \label{fig:factory_goal_tools}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/toolnet/home_world_tools.pdf}
        \caption{Home domain}
        \label{fig:home_world_tools}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/toolnet/factory_world_tools.pdf}
        \caption{Factory domain}
        \label{fig:factory_world_tools}
    \end{subfigure}
    \caption{\footnotesize{\textbf{Diversity of tool usage in human demonstrated plans. } The distribution of tool usage count of top 10 tools with associated goals/scenes in the dataset. Human instructed plans show diversity in 
    the use of tools for the robot to attain the intended goals or environmental contexts.}}
    \label{fig:tool_with_goals}
\end{figure}
%
\begin{figure}[!b]
    \centering
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figures/tango/planlen.pdf}
        \caption{Number of plans}
        \label{fig:plan_len}
    \end{subfigure}
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figures/num_actions.pdf}
        \caption{Symbolic actions}
        \label{fig:num_actions}
    \end{subfigure}
    \caption{\footnotesize{\textbf{Dataset Characteristics: } Distribution of plans with action sequence length. Frequency of actions in both Home and Factory domains for the 10 most frequent action.}}
    \label{fig:dataset}
\end{figure}
%
\begin{figure}[]
    \centering
    % \begin{subfigure}{0.32\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figures/planlen.pdf}
    %     \caption{Number of plans}
    %     \label{fig:plan_len}
    % \end{subfigure}
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figures/num_int.pdf}
        \caption{Object interactions} \vspace{-6pt}
        \label{fig:num_int}
    \end{subfigure}
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figures/num_actions.pdf}
        \caption{Symbolic actions} \vspace{-6pt}
        \label{fig:num_actions}
    \end{subfigure} \setlength{\belowcaptionskip}{-6pt}
    \caption{Data set Characteristics. 
    Distribution of plans with plan length for home and factory domains. Frequency of interaction of top 10 objects and frequency of actions for top 10 actions. 
    The collected data set contains diverse interactions in complex spaces.
    }
    \label{fig:dataset}
\end{figure}
